CosmoDRAGoN II: Remnant Radio Galaxies in Group and Cluster Environments

Radio galaxy remnants are a rare subset of the radio-loud active galactic nuclei (RLAGN) population, representing the quiescent phase in the RLAGN lifecycle. Despite their observed scarcity, they offer valuable insights into the AGN duty cycle and feedback processes. Due to the mega-year timescales over which the RLAGN lifecycle takes place, it is impossible to observe the active to remnant transition in real-time. Numerical simulations offer a solution to follow the long-term evolution of RLAGN plasma. In this work, we present the largest suite (to date) of three-dimensional, hydrodynamic simulations studying the dynamic evolution of the active-to-remnant transition and explore the mechanisms driving cocoon evolution, comparing the results to the expectations of analytic modelling. Our results show key differences between active and remnant sources in both cluster environments and in lower-density group environments. We find that sources in low-density environments can remain overpressured well into the remnant phase. This significantly increases the time for the remnant lobe to transition to a buoyant regime. We compare our results with analytic expectations, showing that the long-term evolution of radio remnants can be well captured for remnants whose expansion is largely pressure-driven if the transition to a coasting phase is assumed to be gradual. We find that remnants of low-powered progenitors can continue to be momentum-driven for about 10 Myr after the jets switch-off. Finally, we consider how the properties of the progenitor influence the mixing of the remnant lobe and confirm the expectation that the remnants of high-powered sources have long-lasting shocks that can continue to heat the surrounding medium.

==> appendices.tex <==
\section{Appendix A - extra plots}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/extra_low_power_particle_plots.png}
    \caption{Extra `particle mixing' section plots for low-powered progenitors}
    \label{fig:extra low powered particle plots}
\end{figure*}


\section{Appendix B - the magnetic field calculations}

Going through \cite{Shabala_sound_waves_2009} and attempting to re-derive the e-folding time for the Perseus cluster. It's given as $5.5\times10^7$ years.\\

\noindent First, listed quantities for the Perseus cluster: 
\begin{table}[H]
    \centering
    \begin{tabular}{l|l|l}
        parameter & physical meaning & given value/equation  \\
        \hline
        g & gravity outside the bubble &  $=-c^2 (d/\gamma r)$ \\
        d & exponent on density profile & 0.76 \\ 
        c & sound speed & $1.17 \times 10^6$ m/s \\ 
        $\gamma$ & ideal gas adiabatic index & 5/3 \\
        $\lambda$ & wavelength & 11 kpc \\
        B & magnetic field strength & $120 \mu G$ \\ 
        A & some dimensionless constant & eq. below \\
        a & bubble radius & 6 kpc \\
        $n_a$ & number density at bubble surface & 0.116 cm$^{-3}$\\
        $\epsilon$ & fractional amplitude term & 0.1 \\
        $\mu$ & dimensionless thing & 0.3 
    \end{tabular}
    \caption{Table of parameters used in \cite{Shabala_sound_waves_2009} equations}
    \label{tab:Shabala 2009 Perseus parameters}
\end{table}

\noindent Want to determine how long the surface of the bubble will remain stable to instability growth. 

\noindent Given the number density at the bubble surface is 0.116 cm$^{-3}$, the mass density can be found from $rho = n \mu m_p$. For $\mu = 0.6$, $rho = 1.17 \times 10^{-25} g / cm^3 $. Seems reasonable.\\

\noindent The largest wave number for any growing
instability is $k_{crit} = [(\rho_{ICM} - \rho_{bubble})g / \sigma]^{1/2}$. If $\rho_{ICM} >> \rho_{bubble}$ then $k_{crit}$ is effectively $ (\frac{\rho_{ICM}g}{\sigma})^{1/2}$. \\

\noindent The effect of a magnetic field alters the surface tension, $\sigma$, and so we have $\sigma = \frac{B}{2\pi \mu_0 k}$ and I'm assuming that $k$ is a wave number given by, 
$$ k \approx \left(\frac{\omega_b - i\beta}{c} \right) + i \frac{d}{2\gamma} $$

\noindent where $(\omega_b - i\beta) / c \sim 2\pi / \lambda$. \\

\noindent \textbf{OR, more usefully}, $k = A/a$ for $A$ given below. Both approaches yield similar values of the order $10^{-20} m^{-1}$. \\

\noindent To determine the `e-folding' time, $t_e = 1 / \omega_{max}$, we need $\omega_{max} = (-g_{eff} k_{crit})^{1/2}$ with the effective gravity $g_{eff}$, given as a combination of the term due to
the gravitational potential of the well, $g_{grav}$, and the acceleration of the oscillating cocoon  $g_{osc}$. So $g_{eff} = g_{grav} + g_{osc}$. The oscillation term, $g_{osc}$, is given by 
$$ g_{osc} = \frac{c^2}{a} \left[ \frac{A^3}{(A^2 + 1)}\right] \left(\frac{\epsilon^2}{(1 + \epsilon)^{3+2d/\gamma}}\right)\left[2 - \left(\frac{2d}{\lambda}\right)\epsilon \right] $$ 

\noindent $g_{grav}$ is given as $c^2(d/(\gamma r))$. 

\noindent Where it's assumed that the oscillations are effectively undamped in order to explain observations. Therefore, the $A$ parameter is that given in S+A09 Eq. 17 and is,

$$A = \left[\frac{6 - \mu + (36 + \mu^2 + 24\mu)^{1/2}}{2\mu}\right]^{1/2}$$. 

\noindent For $mu = 0.3$, $A \sim 4.5$.

\noindent Now, is the $g_{grav}$ parameter calculated using the equation given in the top row of Table \ref{tab:Shabala 2009 Perseus parameters}? Or is it something else? 

\noindent If we assume that $g=-c^2(d/(\gamma r))$, with values in Table \ref{tab:Shabala 2009 Perseus parameters} and $r$ is some radial distance from the potential well. 

At the moment, calculated values for the e-folding time are given in Fig. \ref{fig:efoldtime}.

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Figures/e-folding-time.png}
    \caption{Re-derived values for the e-folding time given in Shabala and Alexander 2009. The value of $5.5\times10^7$ years given in that paper is shown by the grey dashed line.}
    \label{fig:efoldtime}
\end{figure}






